Visually Grounded Continual Learning of Compositional Phrases

Humans acquire language continually with much more limited access to data samples at a time, as compared to contemporary NLP systems. To study this human-like language acquisition ability, we present VisCOLL, a visually grounded language learning task, which simulates the continual acquisition of compositional phrases from streaming visual scenes. In the task, models are trained on a paired image-caption stream which has shifting object distribution; while being constantly evaluated by a visually-grounded masked language prediction task on held-out test sets. VisCOLL compounds the challenges of continual learning (i.e., learning from continuously shifting data distribution) and compositional generalization (i.e., generalizing to novel compositions). To facilitate research on VisCOLL, we construct two datasets, COCO-shift and Flickr-shift, and benchmark them using different continual learning methods. Results reveal that SoTA continual learning approaches provide little to no improvements on VisCOLL, since storing examples of all possible compositions is infeasible. We conduct further ablations and analysis to guide future work.

==> abs_backup.tex <==

\begin{abstract}
%Continual learning algorithms aim at training neural networks over an evolving stream of data without significant forgetting. Existing benchmarks for continual learning usually rely on simple image classification tasks such as handwritten digit classification. These overly simplified testbeds may not fit the goal of deploying continual learning systems in real environments where humans see and learn. 
% Children's language acquisition is a real-world example of continual learning from dynamically evolving visual scenes; yet the community lacks of a properly formalized task and datasets to study such capability.
%the ability state-of-the-art models in learning form dynamic environments.
% The current paradigm of learning compositional semantics using large pre-trained language models requires large memory consumption
Compared to human language acquisition, offline (pre-)training of neural language models (e.g., BERT) demands large memory.
In this paper, we present \vcoll, a visually grounded language learning problem, which simulates the continual acquisition of compositional phrases from visual scenes.
Essentially, \vcoll{} compounds the challenges of \textit{continual learning} and \textit{compositional generalization}.
Models learn from a paired image-caption stream which has continuously shifting object distribution.
They are evaluated throughout the training process by visually-grounded masked language prediction on a regular test set and a held-out test set containing novel phrases of encountered words.
Experiments with state-of-the-art visual-language transformers 
on two constructed datasets COCO-shift and Flickr-shift reveals that \vcoll{} is far from solved, 
and poses new problems than existing continual learning benchmarks. 

% current paradigm of 

% Given image-text pairs, we adopt masked language prediction to evaluate the capability of phase acquisition. Baseline models are first trained on an image-text stream that has continuously shifting object distribution, and later evaluated on a held-out test set with balanced object distribution.
% The proposed task let models 

% coped with different continual learning algorithms 

% It evaluates the models throughout the training process by visually-grounded masked language prediction on a regular test set and a held-out test set that has novel phrases of seen words.
% Our experiments on two constructed datasets, COCO-shifted and Flicker30k-shfited, show that SoTA models, even with memory augmentation, perform far from satisfactory. 
% We construct two image-caption datasets, COCO-shift and Flicker30k-shift, for simulating the continuous data stream.


% classification 
% Compared to classification benchmarks on continual, \vcoll{} presents new challenges.
% a large gap exists between offline-training and continual learning algorithms.
% show performance gaps as compared to offline batch learning.
%Further analysis reveals that generalization to compositional phrases require significantly larger memory for effective continual model learning
%~\footnote{Our code and data can be found at \url{https://github.com/INK-USC/VisCOLL}.}.
\end{abstract}


==> figures/legacy/composition_pairs_fig.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/pair_viz.pdf}
    \vspace{-0.5cm}
    \caption{\small \textbf{Statistics on the compositions of selected adjective and noun in COCO captions.} The large space and biased nature of compositionality are the major challenges of visually  grounded language learning. The novel compositions are filled with gray color.
%     \xisen{as I mentioned in DM, this figure should include discrepancies between train and test combinations to highlight the challenge of the compositional generalization, but regular train and test split won't have much difference between two. I actually think this figure is not necessary} 
%   \junyi{Re: Maybe can show the composition discrepency in the middle of training stream, instead of training set vs. test set}
   }
    \label{fig:pairs}
\end{figure}


==> intro_backupMay31.tex <==
\section{Introduction}
% Children's language acquisition process from the visual world is a real-world example of learning complicated natural language processing tasks. 
% Simulating children's language learning process with neural networks helps researchers to understand the capability and the limit of neural networks~\cite{lake2017generalization, Li2020Compositional}, and inspire researchers deploy them in real-world scenarios, which has drawn interest from vision and language tasks~\cite{bambach2018toddler, Lu2018Neural}.
Learning compositional semantics involves combining atomic words to represent meanings \cite{zadrozny1992compositional} \arka{Need to replace meanings with something more precise}.
It is a fundamental natural language processing task \arka{needs confirmation if indeed a fundamental task/aim}
and has wide applications in \arka{2-3 words on applications, each with 1 citation}.

While pre-trained language models \cite{Devlin2019BERTPO,radford2019language} have shown promising results on compositional semantics \arka{Needs citation, could also add another method}, the current paradigm of offline training relies on large memory computation.
In contrast, humans can learn from streaming data requiring small memory footprint \arka{need psych papers to cite}.
In particular, humans ground visual experience to semantically interpret symbols in a language \cite{harnad1990symbol}.
Inspired by these findings on human language acquisition, we propose \vcoll: a visually grounded continual learning setup to acquire compositional semantics.
As an end-task, we use masked token prediction given an image and a caption with masked noun-phrases (Section \ref{ss:task_def}).
\arka{previous sentence needs paraphrasing}
We illustrate this in Figure \ref{fig:task}.

%%% NEW PARAGRAPH ON PREVIOUS RELEVANT EFFORTS

\begin{figure}[]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/fig_vgmlm_task.pdf}
    \caption{\small \textbf{Visually grounded Continual Compositional Language Learning (VisCOLL).}  We highlight the noun phrase to be masked in each caption. Given image and masked caption, the model is required to predict the masked noun phrase.}
    \label{fig:task}
\end{figure}



\begin{figure*}
    \centering
    \hspace{-0.2cm}
    \includegraphics[width=\textwidth]{figs/fig_double.pdf}
    \vspace{-0.4cm}
    \caption{\small \textbf{Training and testing examples in our problem formulation.} At training, the model visits a stream of image-caption pairs. We highlight the words that are masked for prediction. The distribution of the training data stream, identified by tasks labels, changes continuously over time. See Figure~\ref{fig:stream} for an illustration of the continuous shift. At testing, the model is asked to predict either a seen composition of words or novel composition of seen words.}
    \label{fig:dataset}
\end{figure*}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig_compa.pdf}
    \caption{\small \textbf{Comparison between setups of existing works on continual learning and ours (VisCOLL).}}
    \label{fig:compare}
\end{figure}

%%% another figure to add

% However, no prior work encodes an important challenge for simulating language learning from the visual world: the ability to learn in an evolving environment, also known as continual learning. Previous works on continual learning are usually studied in the context of basic image classification tasks.
%, which are far from the much more realistic and complex setups, such as language acquisition. 

\vcoll{} poses two related challenges.
First, note that unlike previous continual learning works on image classification \arka{need 1-2 citations}, \vcoll{} requires jointly predicting a noun and a verb or adjective which contributes to a significantly larger search space.
As a result of this increased search space, memory based continual algorithms ~\cite{Robins1995CatastrophicFR} cannot expect to store prototypes of each visited compositions.
Second, the increased search space further implies that it is infeasible to view all possible combinations of atomic words at train time.
Therefore, models trained on \vcoll{} should generalize to novel compositions at test time ~\cite{lake2017generalization, keysers2020measuring}.
This is further complicated if the training stream is imbalanced over time.
% \arka{Could/should add imbalanced training stream here as well.}

% composition generalization and catastrophic forgetting which are inherited from language learning and continual learning respectively.
% Arka: Draft {
% describe the challenges precisely (para3)
% describe  
%}

% Continual learning of language modeling is more challenging because of \textit{compositionality}: atomic words can be combined to infinite compositions of words to represent meanings~\cite{zadrozny1992compositional}. For example, memory based continual learning algorithms~\cite{Robins1995CatastrophicFR} should never expect to store prototypes of each visited compositions in a limited memory like label classification. 

% Besides, acquiring compositionality itself is a goal of language learning. 
% Recent study evaluates compositionality learned in models with \textit{compositional generalization}~\cite{lake2017generalization, keysers2020measuring}: at the test phase, the model visits novel composition of inputs or outputs of seen atoms at training. 
% We expect the model to acquire compositionality continuously even when the training stream is imbalanced over time.

% Another challenge that we consider is compositionality in language. Compositionality allows represention of complicated semantics by combining atomic words~\cite{zadrozny1992compositional}. For humans, the ability of handling compositionality emerges as early as 3 years old~\cite{pinker1987productivity,berko1958child}. To test models' ability to learn compositionality, as known as compositional generalization, we formulate the language acquisition problem as a visually grounded masked language modeling task, which requires the model to predict multiple masked words; specifically, we expect the models to compose atomic words to generate novel composition of words. Technically, it also introduces an exponentially large output space, which brings extra challenges for most of the continual learning algorithms. For example, memory based continual learning algorithms, which identify and store important examples for each class in a fixed-sized memory for future replay, should never expect to store an example for each word combination visited. It implies learning the compositionally generalize, \textit{i.e.}, learning to identify atomic concepts in an example and combine them~\cite{keysers2020measuring} is crucial for performance. For example, after storing examples for ``red cars'', ideally the models do not further need to store examples for ``red apples'' to alleviate the forgetting on predicting ``red'' in ``red apples''; in contrast, we do not hope the models overfit the stored examples for ``red cars' by predicting all cars as red or only ``red'' for apples. 
% However, no prior works study such interaction between memory based continual learning and compositional generalization.

% The main contribution of the paper is that we propose a realistic setup aiming at simulating children's language learning process, which encodes both the challenges of continual learning and compositionality. We propose methods to construct the data stream and metrics for evaluation. We test the performance of memory based continual learning algorithms in our setup and also study the interaction between compositional generalization and these algorithms. We show our problem setup is challenging for existing memory based continual learning algorithms, and concluExde that they may cause both overfitting and compositional overfitting, which points out a direction that future works may deal with.


In this work, we extensively study the above challenges associated with \vcoll.
First, we propose final perplexity and averaged perplexity metrics to quantify the performance and forgetfulness of models respectively.
To compute compositional generalization, we further evaluate using novel test splits (details in Section \ref{ss:eval_metrics}).

Second, we construct two datasets with continuously shifting data distribution, namely COCO-shifted and Flickr-shifted.
\arka{Need 1 line on how these are constructed.}
Compared to existing continual learning benchmark datasets, our constructed streams resemble the real-world streams with continuously shifting data distribution (details in Section \ref{sec:data}).

Third, we benchmark \vcoll{} using multi-modal language modeling architecture \cite{Tan2019LXMERTLC,Su2020VL-BERT:} which show state-of-art performance on multiple vision-language tasks.
In particular, we don't use any pre-training, instead train on streaming data using continual learning algorithms \cite{Robins1995CatastrophicFR, rolnick2019experience, Aljundi2019OnlineCL} to evaluate their resistance to forgetting and compositional generalization ability (details in Section \ref{sec:exp_setup}).

Our experiments suggests there exists a large gap between offline training and even state-of-art online continual learning algorithms.
Moreover, composition generalization remains a difficult task for even offline-training.
Finally, we find different compositions have different characteristics \arka{can add one example here, also can add some numerical stats if very impressive} (details in Section \ref{sec:main_expt}).

Our contributions are: 
(i) we propose \vcoll{} task aimed at composing atomic words from streaming paired image-caption data
(ii) we benchmark two datasets COCO-shift and Flickr-shift with multi-modal language models 
(iii) we empirically show the challenges associated with \vcoll{}. \arka{The last contribution may need paraphrasing.}

% To study the challenges above, in this paper, we propose the Visually grounded Continual cOmpositional Language Learning \textbf{(VisCOLL)} task, aiming at simulating real-world language learning process from dynamic environments. 
% We take visually grounded masked language modeling task as a proxy for studying language learning (Figure.~\ref{fig:task}). 
% We create two datasets with continuously shifting data distribution, namely COCO-shifted and Flickr-shifted to encode challenges of continual learning and compositionality for VisCOLL. 
% Compared to existing benchmark datasets for continual learning, the created streams better resemble real-world streams with continuously shifting data distribution.
% We test the performance of two SoTA multi-modal language modeling architecture as multiple continual learning algorithms, evaluating their final performance, resistance to forgetting, as well as compositional generalization ability.  
% We conduct systematic evaluations over the VisCOLL datasets to study the difficulties and the characteristics of the task.


% I have read it and address them,  thx
% \arka{Things that could / should be added to the introduction:
% (i) some reason why this task hasn't been attempted yet? Is it because nobody thought of it or are there some inherent challenges associated with the task that is tackled here? I believe, simulating the imbalanced distribution of the streaming data is a key contribution, basically the creation of CoCo-shift and Flickr-shift. This should be highlighted
% (ii) Extending the previous point, we should also bring out the main challenge in this task: image-classification based continual learning assume task boundaries, in this case there is no task boundaries. Also the memory issue, since exhaustively viewing all combinations is not possible.
% }

==> intro_backup_Jun2.tex <==
\section{Introduction}

Studies of Compositional semantics state that
``the meaning of a compound expression is a function of the meaning of its parts'' \cite{montague1974formal,choi2008learning}; a learner that acquires systematic compositionality can produce large numbers of compositions of seen words~\cite{chomsky1965aspects}.
% Recent work \arka{add citation} show promising results on compositional semantics using pre-trained language 
% models inherently learn compositional semantics 
% \arka{can also add some work other than pre-trained LM}.
% and of the syntactic rules by which they are combined
% involves combining atomic words to represent meanings \cite{zadrozny1992compositional} \arka{Need to replace meanings with something more precise}.
% It is a fundamental natural language processing task \arka{needs confirmation if indeed a fundamental task/aim}
%While pre-trained language models \cite{Devlin2019BERTPO,radford2019language} have shown promising results on compositional semantics \arka{Needs citation, could also add another method}, the current paradigm of offline training relies on large memory requirements.

Recent efforts on modeling compositional semantics such as pre-trained language models \cite{Devlin2019BERTPO,radford2019language} rely on offline (batch) training and large memory requirements. In contrast, humans learn from streaming data and require small memory footprint~\cite{mcclelland1995there}.
In his seminal work on ``symbol grounding,'' ~\citet{harnad1990symbol} suggests that humans ground visual experience to semantically interpret symbols in a language.
Inspired by these findings on human language acquisition, we propose \vcoll: a visually grounded continual learning setup to acquire compositional semantics.
% Given an image and a caption with a masked out noun-phrase, the task is to predict the masked tokens.
As an end-task, we employ masked token prediction of captions given associated image in a continual learning setup as illustrated in Figure \ref{fig:task}-(a)
(formal definition in Section \ref{ss:task_def}).
% As an end-task, we use masked token prediction where given an image and a caption with masked noun-phrases (Section \ref{ss:task_def}).
% \arka{previous sentence needs paraphrasing}


%%% NEW PARAGRAPH ON PREVIOUS RELEVANT EFFORTS

% FIGURE MOVED to folder figures/
\input{figures/intro_fig1}

% \begin{figure}[tb]
% \vspace{-0.1cm}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figs/fig_vgmlm_task.pdf}
%     \vspace{-0.7cm}
%     \caption{\textbf{Visually grounded Continual Compositional Language Learning (VisCOLL)}. We highlight the noun phrase to be masked in each caption. Given image and masked caption, the model is required to predict the masked noun phrase.}
%     \label{fig:task}
%     \vspace{-0.2cm}
% \end{figure}
 


% \begin{figure*}
%     \centering
%     \hspace{-0.2cm}
%     \includegraphics[width=\textwidth]{figs/fig_double.pdf}
%     \vspace{-0.4cm}
%     \caption{\small \textbf{Training and testing examples in our problem formulation.} At training, the model visits a stream of image-caption pairs. We highlight the words that are masked for prediction. The distribution of the training data stream, identified by tasks labels, changes continuously over time. See Figure~\ref{fig:stream} for an illustration of the continuous shift. At testing, the model is asked to predict either a seen composition of words or novel composition of seen words.}
%     \label{fig:dataset}
% \end{figure*}


%%% another figure to add

% However, no prior work encodes an important challenge for simulating language learning from the visual world: the ability to learn in an evolving environment, also known as continual learning. Previous works on continual learning are usually studied in the context of basic image classification tasks.
%, which are far from the much more realistic and complex setups, such as language acquisition. 

Our proposed task \vcoll{} captures two related challenges.
First, unlike previous continual learning works on image classification~\cite{kirkpatrick2017overcoming, zenke2017continual}, \vcoll{} requires predicting a noun with a verb or an adjective which contributes to a significantly large search space.
As a result of this increased search space, memory based continual algorithms ~\cite{Robins1995CatastrophicFR} cannot expect to store prototypes of each visited compositions.
Second, the increased search space makes it infeasible to view all possible combinations of atomic words at train time.
Therefore, models trained for \vcoll{} should generalize to novel compositions at test time (also called \textit{composition generalization}) ~\cite{lake2017generalization, keysers2020measuring}.
This is further complicated when the training stream has an imbalanced distribution with respect to time.
% \arka{Could/should add imbalanced training stream here as well.}

% composition generalization and catastrophic forgetting which are inherited from language learning and continual learning respectively.
% Arka: Draft {
% describe the challenges precisely (para3)
% describe  
%}

% Continual learning of language modeling is more challenging because of \textit{compositionality}: atomic words can be combined to infinite compositions of words to represent meanings~\cite{zadrozny1992compositional}. For example, memory based continual learning algorithms~\cite{Robins1995CatastrophicFR} should never expect to store prototypes of each visited compositions in a limited memory like label classification. 

% Besides, acquiring compositionality itself is a goal of language learning. 
% Recent study evaluates compositionality learned in models with \textit{compositional generalization}~\cite{lake2017generalization, keysers2020measuring}: at the test phase, the model visits novel composition of inputs or outputs of seen atoms at training. 
% We expect the model to acquire compositionality continuously even when the training stream is imbalanced over time.

% Another challenge that we consider is compositionality in language. Compositionality allows represention of complicated semantics by combining atomic words~\cite{zadrozny1992compositional}. For humans, the ability of handling compositionality emerges as early as 3 years old~\cite{pinker1987productivity,berko1958child}. To test models' ability to learn compositionality, as known as compositional generalization, we formulate the language acquisition problem as a visually grounded masked language modeling task, which requires the model to predict multiple masked words; specifically, we expect the models to compose atomic words to generate novel composition of words. Technically, it also introduces an exponentially large output space, which brings extra challenges for most of the continual learning algorithms. For example, memory based continual learning algorithms, which identify and store important examples for each class in a fixed-sized memory for future replay, should never expect to store an example for each word combination visited. It implies learning the compositionally generalize, \textit{i.e.}, learning to identify atomic concepts in an example and combine them~\cite{keysers2020measuring} is crucial for performance. For example, after storing examples for ``red cars'', ideally the models do not further need to store examples for ``red apples'' to alleviate the forgetting on predicting ``red'' in ``red apples''; in contrast, we do not hope the models overfit the stored examples for ``red cars' by predicting all cars as red or only ``red'' for apples. 
% However, no prior works study such interaction between memory based continual learning and compositional generalization.

% The main contribution of the paper is that we propose a realistic setup aiming at simulating children's language learning process, which encodes both the challenges of continual learning and compositionality. We propose methods to construct the data stream and metrics for evaluation. We test the performance of memory based continual learning algorithms in our setup and also study the interaction between compositional generalization and these algorithms. We show our problem setup is challenging for existing memory based continual learning algorithms, and concluExde that they may cause both overfitting and compositional overfitting, which points out a direction that future works may deal with.




In this work, we extensively study \vcoll{} and its associated challenges.
To this end, we 
% propose \arka{name of the method or a 1-line description} to 
construct a continuously shifting data distribution to closely resemble real-word data-stream and contribute shifted versions of COCO-captions \cite{Chen2015MicrosoftCC} and Flickr30k-Entities \cite{Plummer2015Flickr30kEC} namely COCO-shift and Flickr-shift.
% (details in Section \ref{sec:data}).
% We apply this to two COCO-captions \cite{Chen2015MicrosoftCC} and Flickr30k-Entities \cite{Plummer2015Flickr30kEC} and contribute their shifted versions, namely COCO-shift and Flickr-shift.
% (details in Section \ref{sec:data}).
Next, we benchmark these datasets using multi-modal language modeling architectures \cite{Tan2019LXMERTLC,Su2020VL-BERT:} which achieve state-of-art performance on multiple vision-language tasks.
In particular, we don't use any pre-training, instead train on streaming data using continual learning algorithms \cite{Robins1995CatastrophicFR, rolnick2019experience, Aljundi2019OnlineCL} and evaluate their resistance to forgetting and compositional generalization ability. 
% (details in Section \ref{sec:exp_setup}).
% Compared to existing continual learning benchmarks, we construct continuously shifting data distribution streams to resemble the real-world data-stream more closely 
% Furthermore, we 
% We then propose two evaluation metrics, namely, final perplexity and averaged perplexity metrics, to quantify the performance and forgetfulness of trained models respectively.
% (details in Section \ref{sec:data}).
% First, we propose two evaluation metrics, namely, final perplexity and averaged perplexity metrics, to quantify the performance and forgetfulness of trained models respectively.
% To quantitatively measure the performance, we use final perplexity and final BLEU scores. 
% We further propose averaged perplexity metrics to capture the forgetfulness of trained models respectively.
We then propose metrics to quantify the performance and forgetfulness of trained models and evaluate on a novel test split to measure compositional generalization as shown in Figure\ref{fig:task}-(b).
% To compute compositional generalization, we evaluate on a  novel test split of COCO \cite{Nikolaus2019CompositionalGI} (details in Section \ref{ss:eval_metrics}).

% Second, we construct two datasets with continuously shifting data distribution, namely COCO-shifted and Flickr-shifted.
% \arka{Optional: 1 line on how these are constructed.}
% Compared to existing continual learning benchmarks, we construct continuously shifting data distribution streams to resemble the real-world data-stream more closely (details in Section \ref{sec:data}).

% Third, we benchmark \vcoll{} using multi-modal language modeling architecture \cite{Tan2019LXMERTLC,Su2020VL-BERT:} which show state-of-art performance on multiple vision-language tasks.
% In particular, we don't use any pre-training, instead train on streaming data using continual learning algorithms \cite{Robins1995CatastrophicFR, rolnick2019experience, Aljundi2019OnlineCL} and evaluate their resistance to forgetting and compositional generalization ability (details in Section \ref{sec:exp_setup}).

Our experiments validate that there is
a substantial gap exists between offline training and state-of-art online continual learning algorithms.
Moreover, composition generalization remains a difficult task for even offline-training.
Finally, we find different compositions have different characteristics with respect to forgetting. % \arka{Optional: can add one example here, also can add some numerical stats if very impressive} (details in Section \ref{sec:main_expt}).
% \arka{If lack of space, the above paragraph can be removed as a whole.}

To summarize, our contributions are: 
%(i) we propose \vcoll{} task aimed at composing atomic words from streaming paired image-caption data
(i) we propose \vcoll{} task aimed at continual learning of compositional semantics from visually grounded text inputs
(ii) we benchmark two datasets COCO-shift and Flickr-shift with multi-modal language models 
(iii) we empirically demonstrate that \vcoll{} is extremely difficult for state-of-art visually grounded masked language models and continual algorithms and analyze the challenges and potential future research direction. %\arka{The last contribution may need paraphrasing.}

% To study the challenges above, in this paper, we propose the Visually grounded Continual cOmpositional Language Learning \textbf{(VisCOLL)} task, aiming at simulating real-world language learning process from dynamic environments. 
% We take visually grounded masked language modeling task as a proxy for studying language learning (Figure.~\ref{fig:task}). 
% We create two datasets with continuously shifting data distribution, namely COCO-shifted and Flickr-shifted to encode challenges of continual learning and compositionality for VisCOLL. 
% Compared to existing benchmark datasets for continual learning, the created streams better resemble real-world streams with continuously shifting data distribution.
% We test the performance of two SoTA multi-modal language modeling architecture as multiple continual learning algorithms, evaluating their final performance, resistance to forgetting, as well as compositional generalization ability.  
% We conduct systematic evaluations over the VisCOLL datasets to study the difficulties and the characteristics of the task.


% I have read it and address them,  thx
% \arka{Things that could / should be added to the introduction:
% (i) some reason why this task hasn't been attempted yet? Is it because nobody thought of it or are there some inherent challenges associated with the task that is tackled here? I believe, simulating the imbalanced distribution of the streaming data is a key contribution, basically the creation of CoCo-shift and Flickr-shift. This should be highlighted
% (ii) Extending the previous point, we should also bring out the main challenge in this task: image-classification based continual learning assume task boundaries, in this case there is no task boundaries. Also the memory issue, since exhaustively viewing all combinations is not possible.
% }

==> intro_old_backup.tex <==
\section{Introduction}
%The ability to continuously learn in an evolving environment is one of the key traits human intelligence exhibits. Neural networks, in contrast, are known to suffer from catastrophic forgetting~\cite{Robins1995CatastrophicFR} of previously learned knowledge. To address the problem, researcher study continual learning algorithms~\cite{parisi2018continual}.
Children's language acquisition process from the visual world is a real-world example of learning complicated natural language processing tasks. 
Simulating children's language learning process with neural networks helps researchers to understand the capability and the limit of neural networks in learning from real-world environments~\cite{suris2019learning}, and inspire researchers to push the limit by addressing the found issues~\cite{Lu2018Neural, lake2017generalization}.

%%% NEW PARAGRAPH ON PREVIOUS RELEVANT EFFORTS

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig_vgmlm_task.pdf}
    \caption{\textbf{Visually grounded Continual Compositional Language Learning (VisCOLL).}  We highlight the noun phrase to be masked in each caption. Given image and masked caption, the model is required to predict the masked noun phrase.}
    \label{fig:task}
\end{figure}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/pair_viz.pdf}
    \caption{\textbf{Statistics on the compositions of selected adjective and noun in COCO captions.} The large space and biased nature of compositionality are the major challenges of visually  grounded language learning. The novel compositions are filled with gray color. \xisen{as I mentioned in DM, this figure should include discrepancies between train and test combinations to highlight the challenge of the compositional generalization, but regular train and test split won't have much difference between two. I actually think this figure is not necessary} 
   \junyi{Re: Maybe can show the composition discrepency in the middle of training stream, instead of training set vs. test set}}
    \label{fig:pairs}
\end{figure}

\begin{figure*}
    \centering
    \hspace{-0.4cm}
    \includegraphics[width=\textwidth]{figs/fig_double.pdf}
    \caption{\textbf{Training and testing examples in our problem formulation.} At training, the model visits a stream of image-caption pairs. We highlight the words that are masked for prediction. The distribution of the training data stream, identified by tasks labels, changes continuously over time. See Figure~\ref{fig:stream} for an illustration of the continuous shift. At testing, the model is asked to predict either a seen composition of words or novel composition of seen words.}
    \label{fig:dataset}
\end{figure*}

%%% another figure to add

However, no prior work encodes an important challenge for simulating language learning from the visual world: the ability to learn in an evolving environment, also known as continual learning. Previous works on continual learning are usually studied in the context of basic image classification tasks, which are far from the much more realistic and complex setups, such as language acquisition. Continual learning of language modeling is more challenging because of \textit{compositionality}: atomic words can be combined to infinite compositions of words to represent meanings~\cite{zadrozny1992compositional}. For example, memory based continual learning algorithms~\cite{Robins1995CatastrophicFR} should never expect to store prototypes of each visited compositions in a limited memory like label classification tasks (Fig. \ref{fig:pairs}).

Besides, acquiring compositionality itself is a goal of language learning. Recent study evaluates compositionality learned in models with \textit{compositional generalization}~\cite{lake2017generalization, keysers2020measuring}: at the test phase, the model visits novel composition of inputs or outputs of seen atoms at training. We expect our models to acquire compositionality even when the training stream is imbalanced over time.

% Another challenge that we consider is compositionality in language. Compositionality allows represention of complicated semantics by combining atomic words~\cite{zadrozny1992compositional}. For humans, the ability of handling compositionality emerges as early as 3 years old~\cite{pinker1987productivity,berko1958child}. To test models' ability to learn compositionality, as known as compositional generalization, we formulate the language acquisition problem as a visually grounded masked language modeling task, which requires the model to predict multiple masked words; specifically, we expect the models to compose atomic words to generate novel composition of words. Technically, it also introduces an exponentially large output space, which brings extra challenges for most of the continual learning algorithms. For example, memory based continual learning algorithms, which identify and store important examples for each class in a fixed-sized memory for future replay, should never expect to store an example for each word combination visited. It implies learning the compositionally generalize, \textit{i.e.}, learning to identify atomic concepts in an example and combine them~\cite{keysers2020measuring} is crucial for performance. For example, after storing examples for ``red cars'', ideally the models do not further need to store examples for ``red apples'' to alleviate the forgetting on predicting ``red'' in ``red apples''; in contrast, we do not hope the models overfit the stored examples for ``red cars' by predicting all cars as red or only ``red'' for apples. 
% However, no prior works study such interaction between memory based continual learning and compositional generalization.

% The main contribution of the paper is that we propose a realistic setup aiming at simulating children's language learning process, which encodes both the challenges of continual learning and compositionality. We propose methods to construct the data stream and metrics for evaluation. We test the performance of memory based continual learning algorithms in our setup and also study the interaction between compositional generalization and these algorithms. We show our problem setup is challenging for existing memory based continual learning algorithms, and concluExde that they may cause both overfitting and compositional overfitting, which points out a direction that future works may deal with.

To study the challenges above, in this paper, we propose the Visually grounded Continual cOmpositional Language Learning \textbf{(VisCOLL)} task, aiming at simulating real-world language learning process from dynamic environments. We take visually grounded masked language modeling task as a proxy for studying language learning (Figure.~\ref{fig:task}). We create two datasets with continuously shifting data distribution, namely COCO-shifted and Flickr-shifted to encode challenges of continual learning and compositionality for VisCOLL. 
We test the performance of two SoTA multi-modal language modeling architecture as multiple continual learning algorithms, evaluating their final performance, resistance to forgetting, as well as compositional generalization ability.  % We conduct systematic evaluations over the VisCOLL datasets to study the difficulties and the characteristics of the task.

\arka{Things that could / should be added to the introduction:
(i) some reason why this task hasn't been attempted yet? Is it because nobody thought of it or are there some inherent challenges associated with the task that is tackled here? I believe, simulating the imbalanced distribution of the streaming data is a key contribution, basically the creation of CoCo-shift and Flickr-shift. This should be highlighted
(ii) Extending the previous point, we should also bring out the main challenge in this task: image-classification based continual learning assume task boundaries, in this case there is no task boundaries. Also the memory issue, since exhaustively viewing all combinations is not possible.
}

==> setup_backup_Jun3.tex <==
\input{figures/main_model_fig}



\section{Methods}
%\arka{should we change the name of the section from models to Method or Experimental setup?}


% \begin{figure*}[tb]
% \vspace{-0.2cm}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figs/mlm_arch.pdf}
%     \vspace{-0.3cm}
%     \caption{\textbf{Architecture of Base Model for VisCOLL.} Image embedding is extracted via ResNet and fed into the model together with the word embeddings of the masked captions. The word embedding layer is randomly initialized.}
%     \label{fig:arch}
% \end{figure*}

% \begin{table*}[]
% \centering
% \scalebox{0.85}{\begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{Dataset}        & \multicolumn{4}{c}{\textbf{COCO-shift}}                                        & \multicolumn{3}{c}{\textbf{Flickr-shift}}                                      \\\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-8}
% \textbf{Method/Metrics} & \textbf{PPL} & \textbf{Noun acc.} & \textbf{Verb acc.} & \textbf{Adj. acc.} & \textbf{PPL} & \textbf{Noun acc.} & \textbf{Adj. acc.} \\ \cmidrule[1pt](){1-8}
% Vanilla Online   & 6.055        & 0.51               & 20.93              & 1.58               & 5.965        &       1.72             &       6.96                                 \\
% Single-pass Offline        & 1.923        & 51.55              & 47.00              & 25.11              & 2.978        &          26.44          &        14.70                                \\ \cmidrule{1-8}
% Experience Reply (ER)             &              &                    &                    &                    &              &                    &                                        \\
% ~$-$~\textit{$|M|$=1,000}        & 4.475        & 14.59              & 33.81              & 7.76               & 5.485        &      3.79              &     7.41                                   \\
% ~$-$~\textit{$|M|$=10,000}       & 3.193        & 33.23              & 42.69              & 18.81              & 4.303        &      15.69              &    13.41                                    \\
% ~$-$~\textit{$|M|$=100,000}      & 2.119        & 45.60              & 49.19              & 25.63              &    3.005          &     26.54               &       18.21                                 \\ \cmidrule{1-8}
% Maximally Interfering Retrieval (MIR)            &              &                    &                    &                    &              &                    &                                        \\
% ~$-$~\textit{$|M|$=10,000}       & 3.186        & 33.60              & 41.79              & 17.49              & 3.688         &       16.67             &           11.57                         \\ \bottomrule
% \end{tabular}}
% \caption{Overall performance of methods in MS COCO dataset and Flickr30k dataset.}
% \label{tab:overall}
% \end{table*}

% \begin{table*}[]
% \centering
% \scalebox{0.66}{
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
% \textbf{Model}                         & \multicolumn{6}{c}{\textbf{VLBERT}}                                                                                                   & \multicolumn{6}{c}{\textbf{LXMERT}}                                                                                            \\ \midrule
% \textbf{Metrics}                       & \multicolumn{2}{c}{\textbf{Final Perplexity ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} \\ \midrule
% \textbf{Memory sizes}                  & \textbf{1,000}        & \textbf{10,000}       & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    & \textbf{1,000}    & \textbf{10,000}    & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    \\ \midrule
% \textbf{iid-online}                    & \multicolumn{2}{c}{1.610}                     & \multicolumn{2}{c}{65.27 / 39.61}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{1.783}              & \multicolumn{2}{c}{61.74 / 36.03}             & \multicolumn{2}{c}{-}                   \\
% \textbf{iid-offline}                   & \multicolumn{2}{c}{1.443}                     & \multicolumn{2}{c}{68.93 / 44.16}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{1.503}              & \multicolumn{2}{c}{67.53 / 42.79}             & \multicolumn{2}{c}{-}                   \\
% \textbf{Vanilla}                       & \multicolumn{2}{c}{5.040}                     & \multicolumn{2}{c}{25.96 / 1.29}              & \multicolumn{2}{c}{0.540}      & \multicolumn{2}{c}{5.193}              & \multicolumn{2}{c}{25.19 / 1.81}              & \multicolumn{2}{c}{0.612}               \\
% \textbf{ER}                            & \textbf{3.152}                 & \textbf{2.307}                 & \textbf{45.80} / 20.50          & 58.06 / 32.22          & 0.026             & -0.142             & \textbf{3.154}             & 2.426              & \textbf{49.52} / \textbf{24.56}          & 61.01 / \textbf{35.45}          & -0.069             & \textbf{-0.154}             \\
% \textbf{AGEM}                          & 3.478                 & 3.269                 & 37.94 / 13.56          & 40.21 / 15.64          & 0.235              & 0.145              & 3.411             & 3.227              & 38.71 / 14.72          & 40.28 / 15.87          & 0.361              & 0.257              \\
% \textbf{ER+MIR}                        & 3.342                 & 2.469                 & \textbf{45.80} / \textbf{20.87}          & 58.00 / 32.33          & 0.012             & -0.133             & 3.162             & \textbf{2.374}              & 48.77 / 23.72          & 60.79 / 35.10          & \textbf{-0.076}             & -0.147             \\
% \textbf{ER+MIR$_{max}$} &        3.344               & 2.473                 &          45.53 / 20.23            & \textbf{58.14} / \textbf{32.48}          &        \textbf{-0.056}            & \textbf{-0.153}             &      3.218             &        2.378        &          48.03 / 23.10            &          \textbf{61.06} / 35.24            &      -0.040              &         -0.140           \\ \bottomrule
% \end{tabular}
% }
% \caption{Final log perplexity, BLEU-1/2 and forgetting metrics on the \textbf{COCO-shifted} dataset. The dash symbol indicates the metrics is not applicable for the method.}
% \label{tab:coco_overall}
% \end{table*}


% \begin{table*}[]
% \centering
% \scalebox{0.66}{
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
% \textbf{Model}          & \multicolumn{6}{c}{\textbf{VLBERT}}                                                                                                   & \multicolumn{6}{c}{\textbf{LXMERT}}                                                                                            \\ \midrule
% \textbf{Metrics}        & \multicolumn{2}{c}{\textbf{Final Perplexity ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} \\ \midrule
% \textbf{Memory sizes}   & \textbf{1,000}        & \textbf{10,000}       & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    & \textbf{1,000}    & \textbf{10,000}    & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    \\ \midrule
% \textbf{iid-online}     & \multicolumn{2}{c}{2.590}                     & \multicolumn{2}{c}{47.08 / 21.88}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{2.640}              & \multicolumn{2}{c}{47.30 / 22.56}             & \multicolumn{2}{c}{-}                   \\
% \textbf{iid-offline}    & \multicolumn{2}{c}{2.025}                     & \multicolumn{2}{c}{57.13 / 32.29}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{2.025}              & \multicolumn{2}{c}{57.10 / 32.25}             & \multicolumn{2}{c}{-}                   \\
% \textbf{Vanilla}        & \multicolumn{2}{c}{5.691}                     & \multicolumn{2}{c}{25.01 / 3.01}              & \multicolumn{2}{c}{0.456}           & \multicolumn{2}{c}{6.107}              & \multicolumn{2}{c}{24.77 / 3.09}              & \multicolumn{2}{c}{0.619}                    \\
% \textbf{ER}             & 5.016                 & \textbf{3.492}                 & \textbf{29.56} / \textbf{7.96}           & 40.23 / 16.80          &        0.229            &       0.023             & 4.949             &         \textbf{3.197}           & 31.32 / 9.58           &      \textbf{44.34} / 20.73          &          0.237          &     0.021       \\
% \textbf{AGEM}           & \textbf{4.493}                 & 4.393                 & 28.43 / 6.52           & 28.97 / 7.35           &         \textbf{0.004}           &      \textbf{-0.056}              & 5.246             & 5.072              & 25.18 / 3.63           & 24.77 / 3.09           &         \textbf{0.108}           &   0.096                 \\
% \textbf{ER+MIR}         & 5.118                & 3.504                 & 29.40 / 7.48           & \textbf{40.27} / \textbf{16.81}          &          0.268          &   -0.020                 & 4.949             & 3.211              & 31.64 / 9.80           & 44.30 / \textbf{20.83}         &       0.188             &     0.001               \\
% \textbf{ER+MIR$_{max}$} & 5.057                 & 3.555                 & 29.43 / 7.51           & 40.04 / 16.64          &         0.233           &       0.009         &     \textbf{4.788}              &    3.226                &        \textbf{31.72} / \textbf{9.89}          &         43.51 / 19.95             &     0.191               &     \textbf{-0.015}               \\ \bottomrule
% \end{tabular}
% }
% \caption{Final log perplexity, BLEU-1/2 and forgetting metrics on the \textbf{Flickr-shifted} dataset. The dash symbol indicates the metrics is not applicable for the method.}
% \label{tab:flickr_overall}
% \end{table*}

% \input{tables/coco_overall_res_tab}
% \input{tables/flickr_overall_res_tab}

\label{sec:exp_setup}
% In this section, we introduce models, continual learning algorithm baselines and metrics for VisCOLL. 

% To analyze \vcoll{} and generate strong baselines, we use two state-of-art base-architectures and train them with state-of-art continual learning algorithms.

In this section, we establish workflows and baselines for VisCOLL. 
We first discuss the choice of base models (Section \ref{ss:base_model}) used for masked token predictions followed by descriptions of continual learning algorithms (Section \ref{ss:cont_algos}) for \vcoll.

% \subsection{Base Model for VisCOLL}
\subsection{Visual Language Encoders}
\label{ss:base_model}
% We modify VLBERT~\cite{Su2020VL-BERT} as our base model. We first encode the image with a ResNet-34~\cite{He2015DeepRL} to get an image embedding. Then, we feed the image embedding as well as the word embeddings of the masked captions into the 4-layer Transformer with a hidden size of 384. The output of the transformer at the masked positions are fed into a linear layer to output the word predictions. We use cross-entropy loss and use Adam~\cite{kingma2014adam} optimizer with a learning rate of 0.0002 throughout the experiments.
Recall that our end-task is masked token prediction where the input is an image and a caption with masked out tokens.
Since the task of masked token prediction is used as a pre-training method in almost all multi-modal masked language models, we choose two such models: VLBERT~\cite{Su2020VL-BERT:} and LXMERT~\cite{Tan2019LXMERTLC} as base models but expect similar conclusions with other models like ViLBERT \cite{Lu2019ViLBERTPT} or UNITER \cite{chen2019uniter}.
For all our experiments, % without pre-trained on any large image-caption dataset like conceptual captions \cite{sharma-etal-2018-conceptual} 
the model weights are randomly initialized, without using any weights from pre-trained language models like BERT \cite{Devlin2019BERTPO}.
%\arka{are the models initialized randomly? if so, could rephrase the previous sentence.}

For both base models, we first extract image and object features in ground truth bounding boxes with a Faster-RCNN~\cite{ren2015faster} model with Resnet-101 backbone ~\cite{He2015DeepRL} pretrained on Visual Genome ~\cite{krishna2017visual} dataset using only object-detection (without attributes).
However, the ground-truth object labels are not provided to the model.
The extracted features are then passed to the base models along with the caption with masked text span replaced with \texttt{[MASK]} tokens, and finally we compute the cross entropy loss. %#at the prediction.
%\arka{Is the loss Cross-Entropy? Then we can just mention it here.}
%\arka{Is there anything differently done at test-time? If so 1-line mention here would be good.}
We illustrate our base model in Figure \ref{fig:arch}.



% on  with detectron2~\cite{wu2019detectron2}. 
% We do not provide ground truth object labels to the model. 
% The features are pre-computed before model training.
% \input{tables/coco_overall_res_tab}
% \input{tables/flickr_overall_res_tab}
% \input{tables/coco_flickr_combined_res_tab}

\subsection{Continual Learning Algorithms}
\label{ss:cont_algos}

%While in the offline-training with i.i.d samples one could simply use stochastic gradient descent algorithms for training in the online continual learning setup this would lead to catastrophic forgetting~\cite{Robins1995CatastrophicFR}.

One could simply use \textbf{Vanilla Online Gradient Descent (Vanilla)} to train models over a data stream, in a similar way to the offline-training setting.
It performs a gradient update on model parameters each time it receives a mini-batch from the training data stream. 
However, it results in significant forgetting~\cite{Robins1995CatastrophicFR}. Thus, using continual learning algorithms a necessity.

We focus on memory based continual learning algorithms for \vcoll, as most of them are scalable to our problem setup, and naturally applicable to the scenarios where no task identifiers are available. Existing approaches from other families, such as regularization based approaches, are shown not to be competitive in complicated setups~\cite{hsu2018re}, but can be explored in future works.

\smallskip
\noindent \textbf{Experience Replay (ER)}~\cite{Robins1995CatastrophicFR, rolnick2019experience} randomly stores visited examples in a fix-sized memory called the replay memory.
At each training iteration, it randomly samples a small mini-batch of examples from the replay memory for retraining. 
To determine which examples to store and replace from the memory, we use reservoir sampling~\cite{vitter1985random}.

\smallskip
\noindent \textbf{Average Gradient Episodic Memory (AGEM)} ~\cite{chaudhry2018efficient} is similar to ER in that it 
% Similar to ER, AGEM~\cite{chaudhry2018efficient} 
also randomly stores visited examples in a fixed-sized memory.
However, unlike ER that relies on retraining to alleviate forgetting, 
% AGEM performs constrains the optimization on model parameters: 
AGEM performs a constrained optimization:
at each training step, the gradients of model parameters are projected to a direction where the average loss on a random subset of memory examples does not increase.
    
\smallskip
\noindent \textbf{ER with Maximally Interfering Retrieval (ER-MIR)}. ER-MIR~\cite{Aljundi2019OnlineCL} is built upon ER.
At each training iteration, instead of randomly sampling a mini-batch to replay, ER-MIR selects examples that are most likely to be forgotten
% for replay 
% by estimating loss increase of memory examples in upcoming updates. 
by estimating the increased loss from memory examples in the next one update.% \arka{Needs confirmation if it is next udpate or next few updates}.

\smallskip
\noindent
\textbf{ER-MIR$_{\mathbf{max}}$}.
% \arka{Should we rename it to ER-MIR(max) instead for clarity?}
We propose a variant of ER-MIR that specifically applies to our compositional prediction setting: instead of averaging forgetting over the masked phrase of an example, we select examples that contain a word that is most likely to be forgotten.
% \arka{Is the word a noun or a verb or could be both. Need 1-line expanding on this.}
% We note the method as \textbf{ER-MIR$_{\mathbf{max}}$}.

%\arka{Should the paragraph below go into Experimental Setup?}


% Besides the continual learning algorithms above, we also report the model performance in \textbf{online i.i.d.} settings and \textbf{offline i.i.d.} settings as two upper bounds. 
\smallskip
\noindent
\textbf{i.i.d Setting}.
To further analyze and set upper bounds on the datasets, we additionally report \textbf{online i.i.d.} settings and \textbf{offline i.i.d.}.
In both settings, the model visits independently and identically distributed (i.i.d.) training examples.
While in the online setting, the model visits training examples for a single pass; in the offline setting, the model is trained for multiple epochs.


% To quantitatively measure compositional generalization, we evaluate the models on a \textit{compositional} test set in additional to the regular test set. The composition test set consists of novel image concept pairs. We ensure the masked positions in the text refer to these novel concept pairs with synonym tables. 

%To measure compositional generalization, we use the compositional test split of COCO dataset introduced in section~\ref{sec:data}. We ensure the masked positions in the caption refer to these novel concept pairs with synonym tables. The perplexity is reported as 


% -- legacy --

% To address the first research question that whether existing continual algorithms are effective in our setting, we employ \textbf{perplexity (PPL)} as the major metrics to measure the general performance of training methods. Throughout the paper, we report the perplexity in the log scale. We also evaluate \textbf{accuracies of noun, verb, adjective predictions} separately. On Flickr-shift dataset, we only include the accuracy of nouns and adjectives as the phrases in the Flickr datasets are noun phrases.

%To address the first research question that whether continual learning algorithms are effective in a large output space, we compare the performance gap between continual learning algorithms and Vanilla/Offline under different memory sizes.

% To address the second research question that how replay memories influence compositional generalization, we start by proposing a measure for compositional overfitting. Given a reference set of compositions $S$, the compositional overfitting of an atomic word $w$ to the set $S$ is measured as the average perplexity difference when $w$ appears in a composition $(w,x)$ in the test set $D_{tt}$ that also exists in $S$, and when $w$ appear in a composition in $D_{tt}$ that does not exist in $S$. Formally, the compositional overfitting is defined as,
% \begin{equation}
%  \begin{split}
%          f_{ovt}(w,S) &= \frac{1}{N_1} \sum_{(w,x) \in D_{tt} - S} PPL(w)  \\
%          &- \frac{1}{N_2} \sum_{(w,x) \in D_{tt} \cap S} PPL(w)
%  \end{split}
% \end{equation}
% We are able to compute compositional overfitting of a word $w$ regarding the replay memory $M$, note as $f_{ovt}(w, M)$. A large $f_{ovt}(w, M)$ implies the perplexity of $w$ is much larger when $w$ appears in compositions that do not exist in the replay memory. We also compute the compositional overfitting of $w$ regarding the training set, noted as $f_{ovt}(w, D_{tr})$. We then compare $f_{ovt}(w, M)$ to a $f_{ovt}(w, D_{tr})$ to evaluate whether the model inclines to overfit combinations stored in the memory more compared to random examples in the training set. We note the difference between $f_{ovt}(w, M)$ and $f_{ovt}(w, D_{tr})$ as $\Delta f_{ovt}(w)$.
% \begin{equation}
%     \Delta f_{ovt}(w) = f_{ovt}(w, M) - f_{ovt}(w, D_{tr})
% \end{equation}
% Recall that we study combinations of nouns and verbs as well as nouns and adjectives. Given a word $w$, we evaluate $d(w)$ for verb-noun composition and adjective-noun composition in the replay memory $M$ separately, noted as $d_v(w)$ and $d_a(w)$. Also note that $w$ can be either an adjective, a noun or a verb. We average $d_v(w)$ over all nouns or verbs, and average $d_a(w)$ over all nouns or adjectives. In this way, we obtain four statistics, noted as $d_{vn}$, $d_{vv}$, $d_{an}$ and $d_{aa}$.




==> tables/coco_overall_res_tab.tex <==

\begin{table*}[]
\centering
\scalebox{0.66}{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\textbf{Model}                         & \multicolumn{6}{c}{\textbf{VLBERT}}                                                                                                   & \multicolumn{6}{c}{\textbf{LXMERT}}                                                                                            \\ \midrule
\textbf{Metrics}                       & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} \\ \midrule
\textbf{Memory sizes}                  & \textbf{1,000}        & \textbf{10,000}       & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    & \textbf{1,000}    & \textbf{10,000}    & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    \\ \midrule
\textbf{iid-online}                    & \multicolumn{2}{c}{1.610}                     & \multicolumn{2}{c}{65.27 / 39.61}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{1.783}              & \multicolumn{2}{c}{61.74 / 36.03}             & \multicolumn{2}{c}{-}                   \\
\textbf{iid-offline}                   & \multicolumn{2}{c}{1.443}                     & \multicolumn{2}{c}{68.93 / 44.16}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{1.503}              & \multicolumn{2}{c}{67.53 / 42.79}             & \multicolumn{2}{c}{-}                   \\
\textbf{Vanilla}                       & \multicolumn{2}{c}{5.040}                     & \multicolumn{2}{c}{25.96 / 1.29}              & \multicolumn{2}{c}{0.540}      & \multicolumn{2}{c}{5.193}              & \multicolumn{2}{c}{25.19 / 1.81}              & \multicolumn{2}{c}{0.612}               \\
\textbf{ER}                            & \textbf{3.152}                 & \textbf{2.307}                 & \textbf{45.80} / 20.50          & 58.06 / 32.22          & 0.026             & -0.142             & \textbf{3.154}             & 2.426              & \textbf{49.52} / \textbf{24.56}          & 61.01 / \textbf{35.45}          & -0.069             & \textbf{-0.154}             \\
\textbf{AGEM}                          & 3.478                 & 3.269                 & 37.94 / 13.56          & 40.21 / 15.64          & 0.235              & 0.145              & 3.411             & 3.227              & 38.71 / 14.72          & 40.28 / 15.87          & 0.361              & 0.257              \\
\textbf{ER+MIR}                        & 3.342                 & 2.469                 & \textbf{45.80} / \textbf{20.87}          & 58.00 / 32.33          & 0.012             & -0.133             & 3.162             & \textbf{2.374}              & 48.77 / 23.72          & 60.79 / 35.10          & \textbf{-0.076}             & -0.147             \\
\textbf{ER+MIR$_{max}$} &        3.344               & 2.473                 &          45.53 / 20.23            & \textbf{58.14} / \textbf{32.48}          &        \textbf{-0.056}            & \textbf{-0.153}             &      3.218             &        2.378        &          48.03 / 23.10            &          \textbf{61.06} / 35.24            &      -0.040              &         -0.140           \\ \bottomrule
\end{tabular}
}
\caption{\textbf{
Comparison of various training algorithms across two base-models on \textbf{COCO-shift}.} We report 
final log perplexity, BLEU-1/2 and forgetting metrics on the \textbf{COCO-shift} dataset. The dash symbol indicates the metrics is not applicable for the method.
}
\label{tab:coco_overall}
\end{table*}


==> tables/flickr_overall_res_tab.tex <==
\begin{table*}[]
\centering
\scalebox{0.66}{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\textbf{Model}          & \multicolumn{6}{c}{\textbf{VLBERT}}                                                                                                   & \multicolumn{6}{c}{\textbf{LXMERT}}                                                                                            \\ \midrule
\textbf{Metrics}        & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final PPL ($\downarrow$)}} & \multicolumn{2}{c}{\textbf{Final BLEU-1/2 ($\uparrow$)}} & \multicolumn{2}{c}{\textbf{Forgetting ($\downarrow$)}} \\ \midrule
\textbf{Memory sizes}   & \textbf{1,000}        & \textbf{10,000}       & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    & \textbf{1,000}    & \textbf{10,000}    & \textbf{1,000}       & \textbf{10,000}      & \textbf{1,000}     & \textbf{10,000}    \\ \midrule
\textbf{iid-online}     & \multicolumn{2}{c}{2.590}                     & \multicolumn{2}{c}{47.08 / 21.88}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{2.640}              & \multicolumn{2}{c}{47.30 / 22.56}             & \multicolumn{2}{c}{-}                   \\
\textbf{iid-offline}    & \multicolumn{2}{c}{2.025}                     & \multicolumn{2}{c}{57.13 / 32.29}             & \multicolumn{2}{c}{-}                   & \multicolumn{2}{c}{2.025}              & \multicolumn{2}{c}{57.10 / 32.25}             & \multicolumn{2}{c}{-}                   \\
\textbf{Vanilla}        & \multicolumn{2}{c}{5.691}                     & \multicolumn{2}{c}{25.01 / 3.01}              & \multicolumn{2}{c}{0.456}           & \multicolumn{2}{c}{6.107}              & \multicolumn{2}{c}{24.77 / 3.09}              & \multicolumn{2}{c}{0.619}                    \\
\textbf{ER}             & 5.016                 & \textbf{3.492}                 & \textbf{29.56} / \textbf{7.96}           & 40.23 / 16.80          &        0.229            &       0.023             & 4.949             &         \textbf{3.197}           & 31.32 / 9.58           &      \textbf{44.34} / 20.73          &          0.237          &     0.021       \\
\textbf{AGEM}           & \textbf{4.493}                 & 4.393                 & 28.43 / 6.52           & 28.97 / 7.35           &         \textbf{0.004}           &      \textbf{-0.056}              & 5.246             & 5.072              & 25.18 / 3.63           & 24.77 / 3.09           &         \textbf{0.108}           &   0.096                 \\
\textbf{ER+MIR}         & 5.118                & 3.504                 & 29.40 / 7.48           & \textbf{40.27} / \textbf{16.81}          &          0.268          &   -0.020                 & 4.949             & 3.211              & 31.64 / 9.80           & 44.30 / \textbf{20.83}         &       0.188             &     0.001               \\
\textbf{ER+MIR$_{max}$} & 5.057                 & 3.555                 & 29.43 / 7.51           & 40.04 / 16.64          &         0.233           &       0.009         &     \textbf{4.788}              &    3.226                &        \textbf{31.72} / \textbf{9.89}          &         43.51 / 19.95             &     0.191               &     \textbf{-0.015}               \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Final log perplexity, BLEU-1/2 and forgetting metrics on the \textbf{Flickr-shift} dataset.} The dash symbol indicates the metrics is not applicable for the method.}
\label{tab:flickr_overall}
\end{table*}

